Type II supernova spectral diversity II: Spectroscopic and photometric correlations

We present an analysis of observed trends and correlations between a large range of spectral and photometric parameters of more than 100 type II supernovae (SNe~II), during the photospheric phase. We define a common epoch for all SNe of 50 days post-explosion where the majority of the sample is likely to be under similar physical conditions. Several correlation matrices are produced to search for interesting trends between more than 30 distinct light-curve and spectral properties that characterize the diversity of SNe~II. Overall, SNe with higher expansion velocities are brighter, have more rapidly declining light-curves, shorter plateau durations, and higher $^{56}$Ni masses. Using a larger sample than previous studies, we argue that `$Pd$' - the plateau duration from the transition of the initial to `plateau' decline rates to the end of the `plateau' - is a better indicator of the hydrogen envelope mass than the traditionally used optically thick phase duration ($OPTd$: explosion epoch to end of plateau). This argument is supported by the fact that $Pd$ also correlates with s$_3$, the light-curve decline rate at late times: lower $Pd$ values correlate with larger s$_3$ decline rates. Large s$_3$ decline rates are likely related to lower envelope masses that enables gamma-ray escape. We also find a significant anticorrelation between $Pd$ and s$_2$ (the plateau decline rate), confirming the long standing hypothesis that faster declining SNe~II (SNe~IIL) are the result of explosions with lower hydrogen envelope masses and therefore have shorter $Pd$ values.

==> t_vel.tex <==
#SN	&    VelHaF	Err	&    VelHam	Err	&    VelHb	Err	&    VelFe4	Err	&    VelFe5	ERr	&    VelFe6	Err	&    ScF	Err	&    ScM	Err	&    VelNa	Err	&    VelBa	Err	&    Sc		Err	
1986L	&    6141	710	&    7610	476	&    6647	434	&    4907	245	&    4278	672	&    4373	411	&    4739	456	&    4283	336	&    5455	3486	&    NaN	NaN	&    NaN	NaN	
1988A	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
1990E	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
1990K	&    6879	432	&    7741	426	&    6492	381	&    NaN	NaN	&    4406	298	&    3916	204	&    4844	450	&    4568	239	&    6297	391	&    4434	312	&    4109	238	
1991al	&    7846	496	&    8768	615	&    7689	634	&    4880	244	&    4751	588	&    4940	548	&    5214	261	&    4540	227	&    7728	1176	&    5643	282	&    4120	206	
1992ad	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
1992af	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
1992am	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
1992ba	&    4524	665	&    6209	439	&    5056	374	&    3143	157	&    3368	487	&    3443	483	&    3458	173	&    3304	165	&    4299	847	&    3026	151	&    3044	152	
1993A	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
1993K	&    7067	551	&    7016	358	&    6260	444	&    4863	269	&    3488	1390	&    4358	218	&    4445	222	&    3742	NaN	&    5437	NaN	&    3971	199	&    4024	NaN	
1993S	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
1999br	&    3065	588	&    3590	265	&    3175	243	&    1507	258	&    1749	223	&    1740	305	&    2092	272	&    1527	443	&    1515	759	&    1225	61	&    1885	94	
1999ca	&    6957	348	&    7285	364	&    6763	338	&    NaN	NaN	&    5565	278	&    5147	257	&    6042	302	&    5673	284	&    6749	337	&    5778	289	&    5001	250	
1999cr	&    5428	361	&    5901	323	&    4892	478	&    NaN	NaN	&    3474	195	&    3632	212	&    0		0	&    3883	194	&    4470	224	&    NaN	NaN	&    NaN	NaN	
1999eg	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
1999em	&    5540	622	&    5963	595	&    5656	626	&    3744	187	&    3319	394	&    3444	365	&    3362	168	&    2977	149	&    3769	451	&    3032	152	&    3089	154	
S0210	&    8088	492	&    7851	762	&    6970	619	&    NaN	NaN	&    6770	424	&    4956	326	&    6210	311	&    5325	NaN	&    6735	455	&    NaN	NaN	&    NaN	NaN	
2002ew	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2002fa	&    6121	649	&    7553	435	&    6292	410	&    3545	268	&    3807	337	&    4104	260	&    4134	207	&    3581	179	&    5687	663	&    NaN	NaN	&    NaN	NaN	
2002gd	&    3693	563	&    4109	266	&    3394	703	&    2248	196	&    2716	204	&    2437	236	&    3147	297	&    2988	409	&    3382	273	&    2097	177	&    2404	325	
2002gw	&    5403	474	&    6600	487	&    5252	518	&    3234	329	&    3277	494	&    3600	357	&    3203	345	&    3215	247	&    3865	304	&    3021	211	&    2961	185	
2002hj	&    6469	661	&    7830	532	&    6377	451	&    3411	579	&    3762	338	&    4162	405	&    4609	230	&    3571	220	&    5193	345	&    NaN	NaN	&    NaN	NaN	
2002hx	&    5667	434	&    7964	504	&    6386	554	&    3237	337	&    3485	215	&    3781	284	&    3005	157	&    3600	200	&    5360	477	&    2522	160	&    3197	302	
2002ig	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    0		0	
2003B	&    4565	339	&    6190	622	&    5474	478	&    3186	575	&    3437	297	&    3488	251	&    3621	260	&    3502	307	&    4024	228	&    3323	265	&    3104	188	
2003bl	&    3650	481	&    3928	435	&    3825	326	&    2050	255	&    2332	213	&    2085	190	&    2440	263	&    2445	207	&    2700	582	&    2766	426	&    2256	184	
2003bn	&    5827	638	&    6812	545	&    5630	471	&    3616	265	&    3588	607	&    3588	530	&    3437	302	&    3236	327	&    4048	397	&    3278	300	&    3118	178	
2003ci	&    5594	280	&    7133	357	&    5857	293	&    2991	150	&    3806	190	&    3653	183	&    4724	236	&    4416	NaN	&    5849	292	&    3125	156	&    4222	211	
2003cn	&    4192	293	&    5361	501	&    4488	946	&    2388	119	&    2764	138	&    2685	197	&    2947	147	&    2522	126	&    3809	695	&    2804	140	&    2965	148	
2003cx	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2003dq	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2003E	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2003ef	&    6349	367	&    7606	610	&    4230	494	&    3904	364	&    4092	534	&    4087	516	&    4016	575	&    3714	395	&    4284	484	&    3561	299	&    3615	181	
2003eg	&    7525	725	&    8440	675	&    6632	418	&    NaN	NaN	&    4630	405	&    4691	456	&    4137	207	&    4204	210	&    6912	468	&    3100	320	&    3390	410	
2003ej	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2003fb	&    6628	561	&    7507	625	&    5535	854	&    4021	754	&    4125	738	&    3974	722	&    4122	704	&    3655	677	&    4734	668	&    4547	649	&    3566	627	
2003gd	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2003hd	&    6732	519	&    7750	539	&    5899	717	&    3838	192	&    3930	260	&    3997	289	&    3754	188	&    3373	169	&    4688	234	&    NaN	NaN	&    NaN	NaN	
2003hg	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2003hk	&    6980	349	&    6550	328	&    5628	281	&    4026	201	&    4114	206	&    4131	207	&    NaN	NaN	&    NaN	NaN	&    5712	286	&    NaN	NaN	&    NaN	NaN	
2003hl	&    5569	738	&    6508	462	&    4515	439	&    3934	382	&    3873	287	&    3795	402	&    3762	329	&    3758	283	&    4492	318	&    3257	252	&    3480	244	
2003hn	&    6521	387	&    6935	462	&    5288	442	&    3433	281	&    3404	249	&    3462	379	&    3445	286	&    3129	293	&    4437	339	&    3573	189	&    3020	375	
2003ho	&    7367	755	&    8200	520	&    6041	302	&    3442	172	&    3715	186	&    3963	198	&    4278	214	&    3943	197	&    4969	248	&    NaN	NaN	&    NaN	NaN	
2003ib	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2003ip	&    7953	486	&    8508	533	&    6736	388	&    NaN	NaN	&    5342	341	&    4501	309	&    5717	286	&    5015	251	&    6432	413	&    4818	241	&    5289	264	
2003iq	&    5893	741	&    7389	386	&    5432	350	&    4223	211	&    4183	225	&    4297	216	&    4142	207	&    3909	195	&    5080	360	&    3720	186	&    3894	195	
2003T	&    5933	403	&    6873	634	&    4010	226	&    3941	341	&    3783	218	&    3870	276	&    3754	190	&    3370	222	&    3968	292	&    4193	257	&    4012	240	
2004dy	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2004ej	&    5471	501	&    6291	429	&    5340	600	&    3513	505	&    3419	307	&    3282	221	&    3534	536	&    3272	319	&    3978	326	&    2866	191	&    3160	223	
2004er	&    8210	582	&    9508	549	&    7774	600	&    5980	427	&    5349	386	&    5174	436	&    5451	311	&    3353	470	&    5716	506	&    5243	634	&    5259	475	
2004fb	&    6604	636	&    7602	444	&    5827	435	&    3900	283	&    4198	425	&    4149	300	&    4335	217	&    3726	186	&    4760	340	&    5217	261	&    3780	410	
2004fc	&    5584	645	&    6269	976	&    4027	329	&    3667	236	&    3652	291	&    3559	256	&    3736	270	&    3569	261	&    4165	541	&    3178	229	&    3373	266	
2004fx	&    4816	525	&    5671	446	&    4164	318	&    2375	206	&    2687	209	&    2772	401	&    2986	177	&    3367	168	&    2870	389	&    3162	158	&    2449	133	
2005af	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2005an	&    8212	888	&    7561	494	&    5295	1497	&    4324	219	&    4301	325	&    3985	303	&    4716	289	&    4517	293	&    4698	1106	&    NaN	NaN	&    3563	178	
2005dk	&    6808	531	&    7823	470	&    6805	359	&    4506	312	&    4500	289	&    4567	306	&    4384	311	&    3911	329	&    6251	709	&    5067	457	&    4012	256	
2005dn	&    8304	672	&    9353	576	&    7518	484	&    2351	118	&    5690	1511	&    4674	434	&    NaN	NaN	&    4818	241	&    6448	627	&    NaN	NaN	&    NaN	NaN	
2005dt	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2005dw	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2005dx	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2005dz	&    6112	595	&    7496	434	&    5873	430	&    NaN	NaN	&    3901	499	&    4072	310	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2005es	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2005J	&    6285	755	&    8317	668	&    6311	404	&    4204	273	&    4099	406	&    4192	437	&    4122	402	&    4159	265	&    4953	386	&    4069	297	&    4548	272	
2005K	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2005lw	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2005me	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2005Z	&    8419	661	&    9332	582	&    7777	843	&    5620	281	&    5593	384	&    5151	411	&    5581	489	&    5387	359	&    7417	560	&    NaN	NaN	&    NaN	NaN	
2006ai	&    6871	821	&    7388	559	&    6235	560	&    4104	353	&    4390	427	&    4587	340	&    4363	258	&    3358	526	&    6120	434	&    NaN	NaN	&    NaN	NaN	
2006bc	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2006be	&    6857	474	&    7531	625	&    5925	755	&    3763	742	&    3851	738	&    4031	722	&    3907	694	&    3337	677	&    4378	668	&    4933	620	&    NaN	NaN	
2006bl	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2006ee	&    5323	426	&    5164	675	&    3004	619	&    3195	254	&    3108	194	&    3008	255	&    3085	299	&    2695	316	&    3221	267	&    2721	262	&    2725	202	
2006it	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2006iw	&    6857	671	&    7531	566	&    6172	694	&    4630	687	&    4310	678	&    4389	722	&    3898	688	&    3451	682	&    5196	724	&    NaN	NaN	&    NaN	NaN	
2006ms	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2006qr	&    5507	419	&    6432	487	&    5060	285	&    3147	872	&    3571	221	&    3621	200	&    3756	188	&    3508	175	&    4804	954	&    3770	188	&    2917	146	
2006Y	&    7671	619	&    8876	589	&    6879	464	&    3724	186	&    4904	731	&    5033	546	&    NaN	NaN	&    NaN	NaN	&    6922	613	&    NaN	NaN	&    NaN	NaN	
2007aa	&    5057	539	&    5925	550	&    4233	374	&    3131	398	&    3161	378	&    3131	396	&    3082	324	&    2865	266	&    3839	321	&    2685	187	&    2893	267	
2007ab	&    8378	505	&    9614	600	&    8094	405	&    NaN	NaN	&    7056	353	&    4737	237	&    6878	344	&    6350	318	&    7198	404	&    6743	337	&    5949	NaN	
2007av	&    6007	338	&    7146	402	&    5320	311	&    3641	182	&    3849	192	&    3821	191	&    3822	191	&    3691	185	&    3935	605	&    3638	182	&    3432	172	
2007bf	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2007hm	&    6132	383	&    8126	544	&    6336	432	&    4258	213	&    4012	201	&    4371	515	&    4796	240	&    3322	166	&    5232	262	&    NaN	NaN	&    NaN	NaN	
2007il	&    7298	809	&    7917	482	&    5855	505	&    4189	281	&    4071	481	&    4250	383	&    NaN	NaN	&    NaN	NaN	&    4759	769	&    NaN	NaN	&    NaN	NaN	
2007it	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2007ld	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2007oc	&    6990	492	&    6675	435	&    5193	436	&    2265	198	&    3262	315	&    3670	343	&    4158	480	&    3832	378	&    4977	450	&    2872	218	&    3247	291	
2007od	&    7080	655	&    7087	428	&    6623	545	&    NaN	NaN	&    5143	363	&    3838	300	&    NaN	NaN	&    3851	193	&    6139	427	&    5100	525	&    4806	240	
2007P	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2007sq	&    8293	1243	&    8186	437	&    7319	366	&    5270	390	&    5203	260	&    5301	265	&    4937	247	&    4107	205	&    5609	280	&    NaN	NaN	&    NaN	NaN	
2007U	&    7308	1137	&    7932	516	&    6831	721	&    NaN	NaN	&    5489	274	&    5388	550	&    5864	293	&    5379	269	&    6410	340	&    NaN	NaN	&    NaN	NaN	
2007W	&    4093	9357	&    4712	558	&    3182	269	&    2333	182	&    2600	337	&    2426	454	&    2531	156	&    2494	164	&    2606	186	&    2078	104	&    2473	124	
2007X	&    8301	675	&    8476	537	&    6609	601	&    NaN	NaN	&    5416	383	&    4585	762	&    6272	399	&    5503	354	&    6107	1008	&    5115	427	&    4978	496	
2007Z	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2008ag	&    6218	463	&    6826	426	&    4546	473	&    4017	292	&    3924	324	&    3912	311	&    3837	326	&    3500	283	&    4185	426	&    3205	230	&    3478	233	
2008aw	&    7684	621	&    8145	1011	&    6567	530	&    4689	376	&    4684	526	&    4497	654	&    4983	458	&    4395	372	&    6366	478	&    4508	394	&    4424	271	
2008bh	&    7177	688	&    7724	430	&    6232	375	&    4205	210	&    4308	232	&    4163	637	&    4295	215	&    4150	207	&    4648	378	&    4433	222	&    3963	198	
2008bk	&    3294	390	&    4086	707	&    2390	224	&    1860	133	&    2247	153	&    2896	460	&    2256	276	&    2426	310	&    2011	171	&    1840	137	&    1991	180	
2008bm	&    1115	56	&    1760	88	&    1382	69	&    1555	78	&    1644	82	&    1274	64	&    NaN	NaN	&    NaN	NaN	&    1756	88	&    NaN	NaN	&    NaN	NaN	
2008bp	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2008br	&    3659	491	&    4043	258	&    2474	169	&    1659	178	&    1826	142	&    1628	218	&    2152	108	&    2535	127	&    1915	96	&    1382	69	&    1666	83	
2008bu	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2008F	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2008ga	&    6400	589	&    7313	653	&    5357	768	&    3307	754	&    3390	732	&    3253	757	&    4665	694	&    3179	677	&    4785	663	&    NaN	NaN	&    NaN	NaN	
2008gi	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2008gr	&    8247	752	&    8705	435	&    7454	385	&    NaN	NaN	&    5364	268	&    4971	249	&    5860	293	&    5521	276	&    7393	708	&    NaN	NaN	&    NaN	NaN	
2008H 	&    6811	790	&    6537	703	&    5308	941	&    3838	420	&    3766	360	&    3714	350	&    3797	400	&    3655	783	&    4633	760	&    3370	325	&    3410	410	
2008hg	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2008ho	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2008if	&    8588	1126	&    8415	549	&    7137	642	&    3182	200	&    4887	298	&    4718	398	&    5018	272	&    4745	251	&    7309	633	&    3789	189	&    4582	234	
2008il	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2008in	&    4384	721	&    4245	768	&    3210	310	&    2754	259	&    2824	373	&    2817	455	&    2666	283	&    2667	251	&    2907	1581	&    2368	203	&    2562	227	
2008K	&    7882	619	&    7784	793	&    6791	701	&    NaN	NaN	&    6134	352	&    5311	437	&    0		0	&    5491	301	&    6984	501	&    NaN	NaN	&    NaN	NaN	
2008M	&    6058	862	&    6793	631	&    5654	474	&    3487	214	&    3436	345	&    3622	458	&    3748	271	&    3593	198	&    4754	1056	&    3368	217	&    3486	275	
2008W	&    5955	665	&    6932	435	&    5815	435	&    3435	335	&    3719	233	&    3820	297	&    3710	224	&    3487	278	&    5197	470	&    3078	255	&    3296	185	
2009aj	&    2787	455	&    3095	183	&    2800	470	&    2082	161	&    2421	197	&    2834	315	&    NaN	NaN	&    NaN	NaN	&    3011	240	&    NaN	NaN	&    NaN	NaN	
2009ao	&    6678	859	&    5920	544	&    5194	471	&    3767	334	&    3672	256	&    3575	210	&    4126	206	&    3745	230	&    4650	335	&    NaN	NaN	&    3396	170	
2009au	&    2601	524	&    2575	215	&    1978	165	&    1613	113	&    1727	161	&    1470	175	&    1769	237	&    1912	296	&    1943	118	&    1285	64	&    1698	85	
2009bu	&    6363	596	&    7316	1521	&    5522	1304	&    3969	267	&    3948	436	&    4007	456	&    4204	210	&    3440	172	&    4448	308	&    NaN	NaN	&    NaN	NaN	
2009bz	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	
2009N	&    4039	377	&    4475	909	&    2799	259	&    2515	282	&    2638	299	&    2588	439	&    2537	238	&    2489	195	&    2692	186	&    2289	206	&    2387	156	
2009W	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	&    NaN	NaN	

